Robust Adaptive Least Squares Polynomial Chaos Expansions in High-Frequency Applications

We present an algorithm for computing sparse, least squares-based polynomial chaos expansions, incorporating both adaptive polynomial bases and sequential experimental designs. The algorithm is employed to approximate stochastic high-frequency electromagnetic models in a black-box way, in particular, given only a dataset of random parameter realizations and the corresponding observations regarding a quantity of interest, typically a scattering parameter. The construction of the polynomial basis is based on a greedy, adaptive, sensitivity-related method. The sequential expansion of the experimental design employs different optimality criteria, with respect to the algebraic form of the least squares problem. We investigate how different conditions affect the robustness of the derived surrogate models, that is, how much the approximation accuracy varies given different experimental designs. It is found that relatively optimistic criteria perform on average better than stricter ones, yielding superior approximation accuracies for equal dataset sizes. However, the results of strict criteria are significantly more robust, as reduced variations regarding the approximation accuracy are obtained, over a range of experimental designs. Two criteria are proposed for a good accuracy-robustness trade-off.

==> arxiv_only/abbreviations.tex <==
%!TEX TS-program = pdflatex
%!TEX root = main.tex
% --------------------
% New Commands
% --------------------



% Domains:
\newcommand{\spatialDomain}{\ensuremath{D}}
\newcommand{\Boundary}{{\ensuremath{\Gamma}}}
\newcommand{\Gzp}{\ensuremath{{\Gamma_{z^+}}}}
\newcommand{\Gzm}{\ensuremath{{\Gamma_{z^-}}}}
\newcommand{\Gyp}{\ensuremath{{\Gamma_{y^+}}}}
\newcommand{\Gym}{\ensuremath{{\Gamma_{y^-}}}}
\newcommand{\Gxp}{\ensuremath{{\Gamma_{x^+}}}}
\newcommand{\Gxm}{\ensuremath{{\Gamma_{x^-}}}}

% Spaces
\newcommand{\R}{\ensuremath{\rm I\!R}}
\newcommand{\Ltwo}{\ensuremath{L^2\left(\spatialDomain\right)}}
\newcommand{\Ltwovector}{\ensuremath{\left(\Ltwo\right)^3}}
\newcommand{\Hcurl}{{\ensuremath{\mathbf{H}\left(\text{curl};\spatialDomain\right)}}}
\newcommand{\Hcurlref}{\ensuremath{\mathbf{H}\left(\text{curl};\hat{\spatialDomain}\right)}}
\newcommand{\Hzerocurl}{\ensuremath{\mathbf{H}_0\left(\text{curl};\spatialDomain\right)}}

% Physical constants
\newcommand{\epsvac}{\ensuremath{\varepsilon_0}}
\newcommand{\muvac}{\ensuremath{\mu_0}}

% Vectors and operators
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\curl}[1]{\ensuremath{\nabla \times #1}}
\renewcommand{\div}[1]{\ensuremath{\nabla \cdot #1}}
\newcommand{\basis}[1]{\ensuremath{\mathbf{w}_{#1}}}
\newcommand*\dif{\mathop{}\!\mathrm{d}}

% Matrices
\newcommand{\stiff}{\ensuremath{\mathbf{K}}}
\newcommand{\mass}{\ensuremath{\mathbf{M}}}

% FEM
\newcommand{\NdofAll}{\ensuremath{{N_h}}}
\newcommand{\NdofRed}{\ensuremath{{N_{\text{DoF}}}}}
\newcommand{\reduced}{\ensuremath{\text{dof}}}


% --------------------
% Acronyms
% --------------------
\newacronym{ae}{a.e.}{almost every}
\newacronym{cad}{CAD}{computer-aided design}
\newacronym{cv}{CV}{cross-validation}
\newacronym{dc}{DC}{downward-closed}
\newacronym{dof}{DoF}{degrees of freedom}
\newacronym{em}{EM}{electromagnetic}
\newacronym{emf}{EMF}{electromagnetic field}
\newacronym{ed}{ED}{experimental design}
\newacronym{fdtd}{FDTD}{finite-difference time-domain}
\newacronym{fe}{FE}{finite element}
\newacronym{fem}{FEM}{finite element method}
\newacronym{gpc}{gPC}{generalized polynomial chaos}
\newacronym{hc}{HC}{hyperbolic cross}
\newacronym{hf}{HF}{high-frequency}
\newacronym{iga}{IGA}{isogeometric analysis}
\newacronym{iid}{iid}{independent and identically distributed}
\newacronym{loo}{LOO}{leave-one-out}
\newacronym{mim}{MIM}{metal-insulator-metal}
\newacronym{nurbs}{NURBS}{non-uniform rational B-splines}
\newacronym{omp}{OMP}{orthogonal matching pursuit}
\newacronym{pec}{PEC}{perfect electric conductor}
\newacronym{pmc}{PMC}{perfect magnetic conductor}
\newacronym{pml}{PML}{perfectly matched layers}
\newacronym{rf}{RF}{radio-frequency}
\newacronym{rhs}{RHS}{right-hand side}
\newacronym{rms}{RMS}{root-mean-square}
\newacronym{rcwa}{RCWA}{rigorous coupled wave analysis}
\newacronym{te}{TE}{transverse electric}
\newacronym{tm}{TM}{transverse magnetic}
\newacronym{tem}{TEM}{transverse electric and magnetic}
\newacronym{sqp}{SQP}{sequential quadratic programming}
\newacronym{svd}{SVD}{singular value decomposition}
\newacronym{lar}{LAR}{least angle regression}
\newacronym{lhs}{LHS}{latin hypercube sampling}
\newacronym{ls}{LS}{least squares}
\newacronym{mlmc}{MLMC}{multilevel Monte Carlo}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{pce}{PCE}{polynomial chaos expansion}
\newacronym{pde}{PDE}{partial differential equation}
\newacronym{pdf}{PDF}{probability density function}
\newacronym[plural=QoIs, firstplural=quantities of interest (QoIs)]{qoi}{QoI}{quantity of interest}
\newacronym{rv}{RV}{random variable}
\newacronym{rdp}{RDP}{random discrete projection}
\newacronym{qmc}{QMC}{quasi Monte Carlo}
\newacronym{td}{TD}{total degree}
\newacronym{tp}{TP}{tensor product}
\newacronym{uq}{UQ}{uncertainty quantification}

% Symbols:
\newcommand{\tp}{^{\!\top}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\def\SymbReg{\textsuperscript{\textregistered}}
\newcommand{\dx}{\ensuremath{{d_x}}}
\newcommand{\dy}{\ensuremath{d_y}}
\newcommand{\dD}{\ensuremath{\,\text{d}D}}
\newcommand{\dB}{\ensuremath{\,\text{d}\Gamma}}
\newcommand{\epsCplx}{\ensuremath{\underline{\epsilon}}}
\newcommand{\interfaceNurbs}{\ensuremath{\vec C}}
\newcommand{\kinc}{\ensuremath{\vec k^\mathrm{inc}}}
\newcommand{\kincX}{\ensuremath{k^{\mathrm{inc}}_x}}
\newcommand{\kincY}{\ensuremath{k^{\mathrm{inc}}_y}}
\newcommand{\kincZ}{\ensuremath{k^{\mathrm{inc}}_z}}
\newcommand{\ktinc}{\ensuremath{\vec k_\mathrm{t}^{\mathrm{inc}}}}
\newcommand{\Einc}{\ensuremath{\vec E^\mathrm{inc}}}
\newcommand{\Esc}{\ensuremath{\vec E^\mathrm{sc}}}
\newcommand{\thetainc}{\ensuremath{\theta^\mathrm{inc}}}
\newcommand{\phiinc}{\ensuremath{\phi^\mathrm{inc}}}
\newcommand{\STMFun}{\ensuremath{S_\mathrm{TM00}}}

% Unit Vectors
\newcommand{\ex}{\ensuremath{\vec e_x}}
\newcommand{\ey}{\ensuremath{\vec e_y}}
\newcommand{\ez}{\ensuremath{\vec e_z}}


% Additional Macros Dimitris
\newcommand{\AdmSet}{\Lambda^{\mathrm{adm}}}

% Additional Macros Armin
\newcommand{\mean}{\mathbb{E}}
\newcommand{\meanMC}{\mathbb{E}_\text{MC}}
\newcommand{\cond}{\zeta}
\newcommand{\var}{\mathbb{V}} 
\newcommand{\varMC}{\mathbb{V}_\text{MC}} 
\newcommand{\cvmax}{\epsilon_\text{cv}}
\newcommand{\cvl}{\epsilon_{\text{cv,}L^2}}
\newcommand{\cvav}{\epsilon_\text{cv,av}}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\todo}[1]{\textcolor{orange}{#1}}
\newcommand{\sampleSet}{\mathcal{Y}}
\newcommand{\modelEval}{\mathcal{B}}
\newcommand{\convMean}{\epsilon_\mean}
\newcommand{\red}[1]{\textcolor{red}{#1}}

% Additional Macros Uli
\newcommand{\modeIndex}{\ensuremath{\alpha}}
\newcommand{\Trace}{\ensuremath{\pi_\text T}}
\newcommand{\trace}{\ensuremath{\pi_\text t}}
\newcommand{\TraceOp}{\text{T}}
\newcommand{\traceOp}{\text{t}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Macros for resolving Gamma symbol clash:
\newcommand{\ImageSet}{\Xi}
\newcommand{\grid}{Z} 

%\newtheorem{definition}{Definition}

%%%%%%%%%%%%%%%%%%
%% Tikz commands %
%%%%%%%%%%%%%%%%%%
%\newcommand{\drawGrid}[2]
%{
%        \foreach \x in {0,1,2,...,#1} {
%            \foreach \y in {0,1,2,...,#1} {
%            	\node at (\x,\y) [square,fill=#2, minimum size=10mm] {};
%%            	\ifnum \y=0
%%            		\ifnum \x>0
%%	            		\node at (\x,\y) [square,below] {$(\x,\y$)};
%%	            	\fi
%%                \fi
%%              	\ifnum \x=0
%%              		\ifnum \y>0
%%	            		\node at (\x,\y) [square,left] {$(\x,\y$)};
%%	            	\fi
%%                \fi
%%              	\ifnum \x=0
%%              		\ifnum \y=0
%%	            		\node at (\x,\y) [square,below left=-1.5mm] {$(\x,\y$)};
%%	            	\fi
%%                \fi                
%            }
%        }
%%% uncomment for grid
%%        \foreach \x in {0,1,2,...,#1} {
%%        	\draw[#2](\x,0) -- (\x,#1);
%%        	\draw[#2](0,\x) -- (#1,\x);
%%        }
%
%
%	% draw axis
%	\draw[thick,->] (-0.5,-0.5) -- (#1+1,-0.5) node[anchor=north west] {$p_1$};
%	\draw[thick,->] (-0.5,-0.5) -- (-0.5,#1+1) node[anchor=south east] {$p_2$};
%	\foreach \x in {0,1,2,...,#1}{
%	    \draw (\x cm,-0.45) -- (\x cm,-0.55) node[anchor=north] {$\x$};
%	}
%	\foreach \y in {0,1,2,...,#1}{
%	    \draw (-0.45,\y cm) -- (-0.55,\y cm) node[anchor=east] {$\y$};
%	}
%}
%
%\newcommand{\drawTP}[2]
%{
%        \foreach \x in {0,1,2,...,#1} {
%            \foreach \y in {0,1,2,...,#1} {
%                \node at (\x,\y) [square,fill=#2, minimum size=10mm] {};
%            }
%        }
%}
%
%\newcommand{\drawTD}[2]
%{
%        \foreach \x in {0,1,2,...,#1} {
%            \foreach \y in {0,1,2,...,#1} {
%				\ifnum \numexpr\x+\y < \numexpr#1+1 
%               		\node at (\x,\y) [circle, fill=#2, minimum size=5mm] {};
%             	\fi 
%            }
%        }
%}
%
%
%\newenvironment{customlegend}[1][]{%
%    \begingroup
%    % inits/clears the lists (which might be populated from previous
%    % axes):
%    \csname pgfplots@init@cleared@structures\endcsname
%    \pgfplotsset{#1}%
%}{%
%    % draws the legend:
%    \csname pgfplots@createlegend\endcsname
%    \endgroup
%}%
%
%% makes \addlegendimage available (typically only available within an
%% axis environment):
%\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}
%
%
%
%\newcommand{\drawCoordinateSystem}[4] % xmin,xmax,ymax,circle
%{
%%% uncomment for grid
%%        \foreach \x in {0,1,2,...,#1} {
%%        	\draw[#2](\x,0) -- (\x,#1);
%%        	\draw[#2](0,\x) -- (#1,\x);
%%        }
%
%
%	% draw axis
%	\draw[thick,->] (#1+#4,0) -- (#2,0) node[anchor=south] {$z$};
%	\draw[thick,->] (#1,#4) -- (#1,#3) node[anchor=north west] {$y$};
%	\draw[thick] (#1,0) circle (#4);
%	\draw[thick] (#1-0.707*#4,-0.707*#4) -- (#1+0.707*#4,0.707*#4){};
%	\draw[thick] (#1-0.707*#4,0.707*#4) -- (#1+0.707*#4,-0.707*#4)node[anchor=south west] {$x$};
%}
%
%
%\pgfmathdeclarefunction{gauss}{2}{%
%  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
%}

